Spectral analysis of continuous FEM for hyperbolic PDEs: influence of approximation, stabilization, and time-stepping

We study continuous finite element dicretizations for one dimensional hyperbolic partial differential equations. The main contribution of the paper is to provide a fully discrete spectral analysis, which is used to suggest optimal values of the CFL number and of the stabilization parameters involved in different types of stabilization operators. In particular, we analyze the streamline-upwind Petrov-Galerkin (SUPG) stabilization technique, the continuous interior penalty (CIP) stabilization method and the local projection stabilization (LPS). Three different choices for the continuous finite element space are compared: Bernstein polynomials, Lagrangian polynomials on equispaced nodes, and Lagrangian polynomials on Gauss-Lobatto cubature nodes. For the last choice, we only consider inexact quadrature based on the formulas corresponding to the degrees of freedom of the element, which allows to obtain a fully diagonal mass matrix. We also compare different time stepping strategies, namely Runge-Kutta (RK), strong stability preserving RK (SSPRK) and deferred correction time integration methods. The latter allows to alleviate the computational cost as the mass matrix inversion is replaced by the high order correction iterations. To understand the effects of these choices, both time-continuous and fully discrete Fourier analysis are performed. These allow to compare all the different combinations in terms of accuracy and stability, as well as to provide suggestions for optimal values discretization parameters involved. The results are thoroughly verified numerically both on linear and non-linear problems, and error-CPU time curves are provided. Our final conclusions suggest that cubature elements combined with SSPRK and CIP or LPS stabilization are the most promising combinations.

==> fourierM.tex <==
The dispersion and the stability properties of numerical methods can be shown \revMR{by means of a spectral analysis. We will focus on the linear case \eqref{eq:conservation_law1}  with periodic boundary conditions:}
%the analytic solution with the weak solution obtained considering the spatial discretization and Continuous Galerkin fomulation with stabilization methods. 
\begin{equation}
    \partial_t u + a \partial_x u = 0, \quad x\in[0,1]
    \label{eq_disp_1}
\end{equation}
%where $a$ is the constant velocity of propagation. In this study, we consider periodic boundary conditions. \\
\revMR{The main idea is to  investigate the semi and fully discrete evolution of periodic waves represented by the 
 %the continous In order to apply the Fourier analysis to
 % \refp{eq_disp_1} %, we test the advection equation on one wave with frequency $\omega$, imposing 
  the ansatz}
\begin{align}
    u &= Ae^{i(kx - \xi t)} = Ae^{i(kx-\omega t)}e^{\epsilon t} \qquad \mbox{with} \quad \xi = \omega + i \epsilon, \quad i=\sqrt{-1}. \label{eq_disp_uex1} 
\end{align}
Here, $\epsilon$ denotes the damping rate, while \revMR{ the wavenumber is denoted by   $k=2\pi/\lambda$  with} $\lambda$ the wavelength. 
\revMR{We recall that the phase velocity defined as} %of a wave is the rate at which a phase of the wave propagates in space. It is generally defined by the relation 
\begin{equation}
    C =  \frac{\omega}{k}.
    \label{eq_PDE_velocity}
\end{equation}
\revMR{represents the celerity with which waves propagate in space, and it is in general a function of the wavenumber.}
Substituting %the ansatz 
\refp{eq_disp_uex1} in the advection equation \refp{eq_disp_1} leads to \revMR{the well known result} %} solution for the exact coefficients
\begin{align}
%    \refp{eq_disp_1}\quad \& \quad \refp{eq_disp_uex1} \quad & \Leftrightarrow \quad -i \xi u + i a K u = 0 \\
%    & \Leftrightarrow \quad -i \omega u + i a K u + \epsilon u = 0 \\    
%    & \Leftrightarrow \quad a =  \frac{w}{K} \quad \mbox{and} \quad \epsilon = 0 \\
    &  \quad C = a \quad \mbox{and} \quad \epsilon = 0.
\end{align}
\revMR{The objective of the next sections is to provide the semi and fully discrete equivalents of the above relations for the finite element methods introduced earlier.
We will consider  polymnomial degrees up tp 4, for all combinations  of different stabilization methods and time integration. This will also allow to investigate the parametric stability wrt
the time step (cfl number) and stabilization parameter. In practice, for each choice we will evaluate the accuracy of the dicrete
  approximation   of  $\omega$ and $\epsilon$,  as well as provide conditions for the non-positivity of    the damping $\epsilon$. For completeness, the study is performed first  in the semi-discrete time continuous case  in
section \ref{sec:fourier_space}. We the consider the fully discrete schemes in section  \ref{sec:fourier_space_time}.}%
%% we compute the analysis when only the spatial discretization is performed, comparing the different stabilization techniques presented before. 
%In Section \ref{sec:fourier_space_time} we perform the complete von Neumann analysis also for different time integration methods, to verify under which conditions the schemes are stable.

% comparison the dispersion without any stabilization and with stabilization, only for the spatial discretization (i.e. continuous in time and discrete in space).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Preliminaries and time continuous analysis}
%Continuous in time and discrete in space}
\label{sec:fourier_space}

%\textcolor{red}{\bf Here we miss completely the equations for the Fourier modes. How are the element coupled. How is the discrete solution represented. How many modes  for a given space ?
%Where is $\theta$ appearing and how ? What is the sytem for the modes? how do we study this system ?  is there any theory/theorem we can apply ? what are we going to look at, what is the physical meaning of the results, what is expected  etc etc }\\

The Fourier analysis for numerical schemes on the periodic domain  is based on Parseval theorem. 
\begin{theorem}[Parseval]
	Let $\hat{u}(k):= \int_{0}^{1} u(x)e^{-i2\pi kx} dx$ for $k\in \mathbb{Z}$ be the Fourier modes of the function $u$. The $\mathbb{L}_2$ norms of the function $u$ and of the Fourier modes coincide, i.e.,
	\begin{equation}
		\int_{0}^{1} u^2(x)dx = \sum_{k\in \mathbb{Z}} |\hat{u}(k)|^2.
	\end{equation}
\end{theorem}
Thanks to this theorem, we can study the amplification and the dispersion of the basis functions of the Fourier space. 
The key ingredient of this study is the repetition of the stencil of the scheme from one cell to another one. \revMR{In particular, }
%Moreover,
 using the ansatz \eqref{eq_disp_uex1} %for the solution, 
 we can  \revMR{write local equations coupling} %recast the
  degrees of freedom belonging to neighbouring cells through a multiplication by \revMR{the factor of  $e^{i\theta}$ representing the shift in space along the oscillating solution. 
  The dimensionless  coefficient
  	\begin{equation}\label{eq_theta}
\theta:=  k\Delta x
	\end{equation}
	is a discrete reduced wave number which naturally appears all along the analysis.
%We notice that the term $\theta:=k\Delta x$ will appear very often in the analysis, that is why we denote it with $\theta$. 
%In fact, there is a sort of equivalence in changing the wave number and the space discretization.
Formally replacing the ansatz in the scheme we end up with a dense  algebraic problem of dimension $p$ (the polynomial degree)  
%In this way, we obtain one equation for each of the $p$ different types of degrees of freedom and they repeat identically for every cell. Hence, the study of a large discretized numerical system, becomes a small system of only $p$ equations for the modes of our linear problem.
reading in the time continuous case }
%In practice we obtain the matrix system, starting with the space discretization of the linear advection equation, 
%in the following way:
\begin{equation}
 \eqref{eq_disp_1}-\eqref{eq_disp_uex1} \quad \Rightarrow \quad - i\xi \mass \mathbf{U}    + a \mathcal{K}_x \mathbf{U} = 0 \label{eq_sys_mat}
\end{equation}
\begin{equation}
\hspace*{-1cm}
    \mbox{with} \quad (\mass)_{ij} = \int_{\Omega} \phi_i \phi_j dx, \qquad (\mathcal{K}_{x})_{ij} = \int_{\Omega} \phi_i \partial_x \phi_j dx + S(\phi_i,\phi_j), 
\end{equation} 
\revMR{with $\phi_j$ the finite element basis functions and $ \mathbf{U} $ the array of all the degrees of freedom. Although system \eqref{eq_sys_mat}   is in general a global eigenvalue problem, we can reduce its complexity by 
using more explicitly ansatz \eqref{eq_disp_uex1}. More exactly, we can introduce elemental vectors of unknowns $\widetilde{\mathbf{U}}^K$ which   for continuous finite elements  is an array of $p$ degrees of freedom
which includes  only one of the two boundary nodes. Using the periodicity of the solution and   denoting by $K\pm1$ the neighbouring elements, we have
\begin{equation}
\widetilde{\mathbf{U}}^{K\pm1} = \widetilde{\mathbf{U}}^{K}e^{\pm\theta}
\label{eq_ad_fourier0}
\end{equation}
This allows to show that  \eqref{eq_sys_mat}  is equivalent to a  compact system (we drop the superscript $^K$ for simplicity)
\begin{equation}
-i\xi \widetilde{\mass}   \widetilde{\mathbf{U}}  + a \widetilde{\mathcal{K}}_x \widetilde{\mathbf{U} }=0
\label{eq_ad_fourier}
\end{equation}
where   the matrices $\widetilde{\mass}$ and $ \widetilde{\mathcal{K}}$ are readily obtained from the elemental discretization matrices by using  \eqref{eq_ad_fourier0}.\\
% linear combinations of the local finite element matrices times    $e^{\pmi\theta}$
%\begin{equation}
%\widetilde{\mass} := M^K
% \partial_t \widetilde{\mathbf{U}}  + a \widetilde{\mathcal{K}}_x \widetilde{\mathbf{U} }=0
%\label{eq_ad_fourier}
%\end{equation}

 As shown in \cite{sherwin_dispersion} some particular cases  can be easily studied analytically.
 For example for the $\mathbb{P}_1$ cG scheme without stabilization one easily finds that}
%As a first example, we show how this evolves in CG context without stabilization, using $\mathbb{P}_1$ elements. The dispersion analysis leads to the coefficients
\begin{equation} 
\frac{\omega}{k} = a \frac{\sin(\theta)}{\theta}\frac{3}{2+\cos(\theta)} \quad \mbox{and} \quad \epsilon = 0.
%\frac{\omega}{k} = a \frac{\sin(\theta)}{\theta}\frac{3}{2+\cos(\theta)} %, \qquad \mbox{with} \quad \theta = k \Delta x. 
%\label{eq_disp_P1}
\end{equation}
%%%%%This can be shown using the ansatz \refp{eq_disp_uex1} for one degree of freedom inside the FE formulation of the transport equation \refp{eq_disp_1}. Indeed,
%%%%%\begin{align}   
%%%%%& -i \xi \frac{e^{-ik \Delta x} +4+e^{ik \Delta x}}{6} u +  a \frac{e^{-ik \Delta x}-e^{ik \Delta x}}{2 \Delta x} u = 0 \nonumber\\
%%%%%     \Longleftrightarrow \quad & \left( -i \xi \frac{2+\cos(\theta)}{3}  +  a \frac{i \sin(\theta)}{ \Delta x} \right) u = 0 \nonumber\\
%%%%%    \Longleftrightarrow \quad &(-i \omega + \epsilon) \frac{2+\cos(\theta)}{3}  +  a \frac{i \sin(\theta)}{ \Delta x}    = 0 \nonumber\\    
%%%%%    \Longleftrightarrow \quad &w = a \frac{\sin(\theta)}{ \Delta x} \frac{3}{2+\cos(\theta)} \quad \mbox{and} \quad \epsilon = 0 \nonumber\\
%%%%%    \Longleftrightarrow \quad &\frac{\omega}{k} = a \frac{\sin(\theta)}{\theta}\frac{3}{2+\cos(\theta)} \quad \mbox{and} \quad \epsilon = 0.
%%%%%\end{align}
%
%\begin{equation}
%\mbox{then, with} \quad \tilde{\mathbb{P}_1} \quad \mbox{elements :} \quad \frac{\omega}{k} = a \frac{\sin(\theta)}{\theta}
%\end{equation}
%
%As show in the last reference, the analysis of more general cases
%For our 1D problem \eqref{eq_disp_1}, the generalization to more degrees of freedom uses a transformation of the local mass matrix $\widetilde{\mass}\in\R^{p\times p}$ and of the derivative matrix $\widetilde{\mathcal{K}_x}\in\R^{p\times p}$, as also shown in \cite{sherwin_dispersion}.

%
%\begin{comment}
% :
%\begin{equation}
%(\mass^l)_{ij} = \int_{K} \phi_i \phi_j dx , \qquad (\mathcal{K}^l_{x})_{ij} = \int_{K} \phi_i \partial_x \phi_j dx 
%\end{equation} 
%Then, considering the definition of $u$ \cref{eq_disp_uex1}, we define $\Tilde{\mass^l} $, $\Tilde{\mathcal{K}^l}_x $ and $\Tilde{\mathbf{U}}$ \cite{sherwin_dispersion} such as in a mesh of degree $P$, $\forall 0 \leq m,n < P$
%\begin{equation}
%(\Tilde{\mass^l})_{[mn]} =  (\mass^l)_{[mn]} + (\mass^l)_{[mP]} e^{+i \theta} \delta_{n0}  + (\mass^l)_{[Pn]} e^{-i \theta} \delta_{m0} + (\mass^l)_{[PP]} \delta_{m0} \delta_{n0}
%\end{equation}
%\begin{equation}
%(\Tilde{\mathcal{K}^l_x})_{[mn]} =  (\mathcal{K}_x^l)_{[mn]} + (\mathcal{K}_x^l)_{[mP]} e^{+i \theta} \delta_{n0}  + (\mathcal{K}_x^l)_{[Pn]} e^{-i \theta} \delta_{m0} + (\mathcal{K}_x^l)_{[PP]} \delta_{m0} \delta_{n0}
%\end{equation}
%And $(\Tilde{\mathbf{U}^l})_i $ the weak solution on the node $i$. \\
%\end{comment}
%
\revMR{As the degree of the approximation increases, so does the size of the eigenvalue problem. For the non stabilized cG in the $\P_2$ we can still find a relatively analytical solution to  associated the quadratic
 equation reading (cf also \cite{sherwin_dispersion})}
%Using this definition, the dispersion analysis can be rewritten as the following eigenvalue problem:
%\begin{equation}
%\widetilde{\mass} \partial_t \widetilde{\mathbf{U}}  + a \widetilde{\mathcal{K}}_x \widetilde{\mathbf{U} }  \quad  \Leftrightarrow \quad \left[ i\xi  - a\widetilde{\mass}^{-1} \widetilde{\mathcal{K}}_x \right] \widetilde{\mathbf{U} } = 0 
%\label{eq_ad_fourier2}
%\end{equation}
%Defining with $\lambda_i(\theta)$ the eigenvalues of \refp{eq_ad_fourier}, $\omega_i(\theta) = \text{Im}(\lambda_i(\theta))$ and $\epsilon_i(\theta) =- \text{Re}(\lambda_i(\theta))$ are the respective phase and damping coefficients of each mode of the solution.  One of these modes is the \textit{principal} one, of which $\omega_i \approx ak$, while the other modes are \textit{parasite} ones that, if not damped properly, can largely affect the quality of the solution. \\
%Solving the eigenvalue system with $\P_2$ elements, we obtain the coefficients
\begin{equation} \hspace{-0.5cm}
\frac{\omega_{1,2}}{k} = a \frac{4\sin(\theta)\pm 2 \sqrt{40\sin^2 (\frac{\theta}{2})-\sin^2(\theta)}}{\theta(\cos(\theta)-3)}.
\end{equation}
For more general cases, the study needs to be performed numerically.  \\

Defining with $\lambda_i(\theta)$ the eigenvalues of \refp{eq_ad_fourier}, $\omega_i(\theta) = \text{Im}(\lambda_i(\theta))$ and $\epsilon_i(\theta) =- \text{Re}(\lambda_i(\theta))$ are the respective phase and damping coefficients of each mode of the solution.  In practice, we solve numerically the eigenvalue problem \eqref{eq_ad_fourier} for $\theta=k \Delta x_p = \frac{2\pi}{N_x}$ varying in $[0,\pi]$, where $N_x$ is the number of the nodes in each wavelength and $\Delta x_p=\Delta x/p$ is the average distance between degrees of freedom.  However, to satisfy the Nyquist stability criterion, it is necessary to have $\Delta x_p \leq \frac{\lambda}{2}$.\\

\revMR{As an example, } in \cref{fig_disp_lag_CT_DS-any} we plot $\omega$ and $\epsilon$ and we see that the Continuous Galerkin (CG) scheme does not have diffusive terms, or, in other words, there is no damping ($\epsilon =0$) in the CG scheme.  
%For all the eigenvalue systems to solve, we obtain one \textit{principal or primary} eigenvalue, which corresponds to the phase $\omega$, and other ones (depending on the size of the system), which correspond to \textit{parasite} modes. 
%These modes can bring a significant loss of accuracy if they are not accompanied by strong damping. 
For clarity of the pictures, we plot in \cref{fig_disp_lag_CT_DS-any} only the principal eigenvalue of each system ($p=1,2,3$) \revMR{\bf How is it defined/computed in practice ?? }. 
As expected, with $\mathbb{P}_1$ elements, the scheme is more dispersive than with $\mathbb{P}_2$/$\mathbb{P}_3$ elements, while, for all of them, there is no dissipation, since the scheme is not stabilized and there is no time discretization. \\


%Below are presented comparisons of relative error depending on type of elements firstly without any stabilization method (see \cref{fig_disp_lag_CT_DS-any}) and the with stabilization method (\cref{fig_disp_lag_CT_DS-lps}); we show a zoom of the area of interest:

%\textbf{NB: } $kh = \pi$ means that $\frac{2\pi}{N_x}  = \pi \quad \Leftrightarrow  \quad N_x = 2$, i.e. the number of point for a wavelength is 2 ($\Delta x = \lambda$). 

\revMR{We apply the same analysis to stabilized methods. The results obtained with SUPG, CIP and LPS stabilizations   lead to an almost identical result shown in Figure \ref{fig_disp_lag_CT_DS-lps}
(reporting the LPS data). The interested reader can  access all the other plots online  \cite{TorloMichel2020git}.  From the  plot  we can see that the increase in polynomial degree
provides the   expected large reduction in dispersion error,   while retaining a small  amount of }
% that the high order schemes are less dispersive than the first order one. 
%Moreover, in the damping plot, we observe that stabilization methods introduce
 numerical dissipation, which permits the damping of \textit{parasite} modes. % and of the dispersed frequencies.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection*{Local Projection Stabilization - LPS :} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%With the LPS stabilization method, the eigenvalues system can be written as follow
%\begin{align}
%	\refp{eq_stab_proj1} \quad \Leftrightarrow & \quad \left[ -i\xi \Tilde{\mass} + a \Tilde{\mathcal{K}}_x +(\Tilde{\mathcal{K}}_{\tau,xx}-\Tilde{\mathcal{K}}_{\tau,x}^T \Tilde{Q}) \right] \Tilde{\mathbf{U} } = 0 \\
%& \qquad \mbox{with} \quad \Tilde{\mass} \Tilde{Q} = \Tilde{\mathcal{K}_x} \Tilde{\mathbf{U} } \\
% \Leftrightarrow & \quad \left[ i\xi - a \Tilde{\mass}^{-1} \left( \Tilde{\mathcal{K}}_x +\tau (\Tilde{\mathcal{K}}_{\tau,xx}-\Tilde{\mathcal{K}}_{\tau,x}^T\Tilde{\mass}^{-1} \Tilde{\mathcal{K}}_x ) \right) \right] \Tilde{\mathbf{U} } = 0
%\end{align}
%And with stablization method, example with the LPS method defines in \refp{eq_stab_proj1}:
\begin{figure}[H]
     \centering
     %\hspace*{-1cm}
     \includegraphics[width=0.9\textwidth]{image_dispersion/disc_space/disp_space_lagrange_any_phase-best.pdf}
     \caption{Phase $\omega$ (left) and amplification $\epsilon$ (right) with \textit{basic} elements without stabilization for $\mathbb{P}_1, \mathbb{P}_2$ and $\mathbb{P}_3$.}
     \label{fig_disp_lag_CT_DS-any}
\end{figure}


\begin{figure}[H]
     \begin{center}
     %\hspace*{-2cm}
     \includegraphics[width=0.9\textwidth]{image_dispersion/disc_space/disp_space_lagrange_LPS_phase-best.pdf}
     \end{center}
     \caption{Phase $\omega$ (left) and amplification $\epsilon$ (right) with basic Lagrange elements with LPS stabilization for $\mathbb{P}_1, \mathbb{P}_2$ and $\mathbb{P}_3$.}
     \label{fig_disp_lag_CT_DS-lps}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection*{Streamline-Upwing/Petrov-Galerkin - SUPG : } \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%With the SUPG stabilization method, the eigenvalues system can be written as follow
%\begin{align}
%	\refp{eq_supg_mat} \quad \Leftrightarrow & \quad \left[ -i\xi \Tilde{\mass} + a \Tilde{\mathcal{K}}_x + (\Tilde{\mathcal{K}}^T_{\tau,x}+\Tilde{\mathcal{K}}_{\tau,xx}) \right] \Tilde{\mathbf{U} } = 0 \\
%	 \Leftrightarrow & \quad \left[ i\xi - a \Tilde{\mass}^{-1} \left( \Tilde{\mathcal{K}}_x + (\Tilde{\mathcal{K}}^T_{\tau,x}+\Tilde{\mathcal{K}}_{\tau,xx} ) \right) \right] \Tilde{\mathbf{U} } = 0
%\end{align}
%
%%\begin{figure}[H]
%%     \centering
%%     \hspace*{-2cm}
%%     \includegraphics[width=19cm]{image_dispersion/disp_space_lagrange_SUPG_relative.png}
%%     \caption{Dispersion analysis, basic elements and SUPG stabilization method}
%%     \label{fig_disp_lag_CT_DS-supg}
%%\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection*{Continuous Interior Penalty - CIP : } \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%With the CIP stabilization method, the eigenvalues system can be written as follow
%\begin{align}
%	\refp{eq_cip_mat} \quad \Leftrightarrow & \quad \left[ -i\xi \Tilde{\mass} + a \Tilde{\mathcal{K}}_x + \Tilde{GJ}_{\tau} \right] \Tilde{\mathbf{U} } = 0 \\
% \Leftrightarrow & \quad \left[ i\xi - a \Tilde{\mass}^{-1} \left( \Tilde{\mathcal{K}}_x + \Tilde{GJ}_{\tau}) \right) \right] \Tilde{\mathbf{U} } = 0
%\end{align}
% 
%%\begin{figure}[H]
%%     \centering
%%     \hspace*{-2cm}
%%     \includegraphics[width=19cm]{image_dispersion/disp_space_lagrange_CIP_relative.png}
%%     \caption{Dispersion analysis, basic elements and CIP stabilization method}
%%     \label{fig_disp_lag_CT_DS-cip}
%%\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Continuous in space and discrete in time}
%
%With RK and SSPRK scheme, we can write 
%\begin{align}
%    U^{(i)} & = \sum_{k=0}^{i-1} \left( \alpha_{ik} U^{(k)} + \Delta t \beta_{ik} L(U^{(k)}) \right), \quad i \in \llbracket 1,m \rrbracket , \quad L(U) = -\partial_x U \nonumber \\
%    U^{(0)} &= U^n, \quad U^{(m)} = U^{n+1}
%    \label{RK}
%\end{align}
%$\alpha_{ij}$ and $\beta_{ik}$ define in \refp{sec_time_scheme}. \\ 
%
%In the case continuous in space and discrete in time, we can also write 
%\begin{align*}
% \refp{eq_disp_1}\quad \& \quad \refp{eq_disp_uex1} \quad  \Rightarrow \quad U^{n+1} & = U^n + \sum_{\alpha=1}^{step} \gamma_{\alpha} (-ika)^\alpha (\Delta t)^\alpha U^n \\
%\mbox{Or} \quad \left| U^{n+1} \right|  = (1 + \sum_{\alpha=1}^{step} \gamma_{\alpha} (-ika)^\alpha (\Delta t)^\alpha) \left| U^n \right| & \quad \Leftrightarrow \quad e^{\epsilon \Delta t } e^{-i\omega \Delta t}  =  (1 + \sum_{\alpha=1}^{step} \gamma_{\alpha} (-ika)^\alpha (\Delta t)^\alpha) = \lambda \\
%\Leftrightarrow \quad \frac{w}{k} & = atan \left( \frac{-\mathbb{I}(\lambda)}{\mathbb{R}(\lambda)} \right)  \frac{1}{k \Delta t}
%\end{align*}
%\begin{figure}[H]
%     \centering
%     \includegraphics[width=13cm]{image_dispersion/disp_time_RK.png}
%     \caption{Dispersion analysis, RK schemes}
%     \label{fig_disp_lag_DT_CS-ssprk3}
%\end{figure}
%\textbf{Remark : } For the \textit{DeC} scheme, if we use cubature elements $\mass^L = \mass$. By developing each corection steps, we finally find that the scheme is equivalent to \textit{RK} scheme.
%\begin{figure}[H]
%     \centering
%     \includegraphics[width=13cm]{image_dispersion/disp_time_RK3.png}
%     \caption{Dispersion analysis, SSPRK3 schemes}
%     \label{fig_disp_lag_DT_CS-ssprk3}
%\end{figure}
%
%\begin{figure}[H]
%     \centering
%     \includegraphics[width=13cm]{image_dispersion/disp_time_RK4.png}
%     \caption{Dispersion analysis, SSPRK4 schemes}
%     \label{fig_disp_lag_DT_CS-ssprk4}
%\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newpage
\subsection{Fully discrete analysis}\label{sec:fourier_space_time}


%\textcolor{red}{\bf Here we must write clearly the cases of RK and DeC; what is the difference ? the matrices for the different methods, or at least 
%their formal expressions should be reported in the appendix. How is the discrete solution represented. How many modes  for a given finite element space ? 
%What is the system for the modes? how do we study this system ?  is there any theory/theorem we can apply ? what are we going to look at, what is the physical meaning of the results, what is expected  etc etc }\\

%In this section 
%The core idea of this analysis is based on the von Neumann stability analysis \cite{LeVeque2007FiniteDM}.
%The difference with Section \ref{sec:fourier_space} is the discrete consideration of the time derivative which leads to a progressive construction of the evolution matrix for the Fourier degrees of freedom.

\subsubsection{Methodology}
We \revMR{analyze now  %perform an analogous dispersion and damping analysis for 
the fully discrete  schemes obtained  using the RK, SSPRK and DeC time marching methods  presented in \cref{sec:timeIntegration}. }
Let us consider as an example the SSPRK schemes \eqref{eq:SSPRKformula}. If we define as $A:=\mass^{-1} \mathcal{K}_x$ we can write the schemes as follows
% RK formulation 1
\begin{equation}
\left  \{
    \begin{array}{ll}
    	\mathbf{U}^{(0)}:= & \mathbf{U}^n \\
        \mathbf{U}^{(s)} := & \sum_{j=0}^{s-1} \left( \gamma_{sj} \mathbf{U}^{(j)} + \Delta t \mu_{sj} A \mathbf{U}^{(j)} \right), \quad s \in \llbracket 1,S \rrbracket \\
	    \mathbf{U}^{n+1}:=&\mathbf{U}^{(S)}.
	\end{array}
    \right .
    \label{eq:discreteSSPRK}
\end{equation}
%In our fully discrete case, the operator $A$ is a matrix defined by $ A = a\M^{-1} \mathcal{K}_x $ with $\M$ and $\mathcal{K}_x$ defined in \cref{eq_Mass_Kx}. % To simplify the notation, we introduce the operator $A =-a\M^{-1} \mathcal{K}_x$, so $ L(U^{(k)}) = -a\M^{-1} \mathcal{K}_x U $.  \\
% RK formulation 2

Expanding all the stages, we can obtain the following formulation:
\begin{equation}
\mathbf{U}^{n+1} = \mathbf{U}^{(0)} + \sum_{j=1}^{S} \nu_{j} \Delta t^jA^j  \mathbf{U}^{(0)} = \left(\mathcal{I} + \sum_{j=1}^{S} \nu_{j}\Delta t^j A^j  \right) \mathbf{U}^n, \label{RK_gamma0}
\end{equation}
where coefficients $\nu_j$ in \eqref{RK_gamma0} are obtained as combination of coefficient $\gamma_{sj}$ and $\mu_{sj}$ in \eqref{eq:discreteSSPRK} and $\mathcal{I} $ is the identity matrix. For example, coefficients of the fourth order of accuracy scheme \textit{RK4} are $\nu_1=1$, $\nu_2 = 1/2$, $\nu_3=1/6$ and $\nu_4 = 1/24$.\\ 
%\begin{comment}
%% continuous in space, d_x U = -ik
%In the case continuous in space and discrete in time, using the definition of $u$ \cref{eq_disp_uex1}, the operator $A$ is a scalar defined by $A U = -a\partial_x U = -aik U$ (i.e. $A =-aik$). We obtain 
%\begin{align}
%U^{n+1} & = U^n + \sum_{\alpha=1}^{step} \gamma_{\alpha} (-ika)^\alpha (\Delta t)^\alpha U^n \label{RK_gamma} \\
%\mbox{Or} \quad \left| U^{n+1} \right|  & = \left(1 + \sum_{\alpha=1}^{step} \gamma_{\alpha} (-ika)^\alpha (\Delta t)^\alpha \right) \left| U^n \right|  \label{RK_gamma_norm} 
%\end{align}
%Then using \eqref{eq_disp_uex1}, $U^{n+1} = U^{n}e^{-i \omega \Delta t} e^{\epsilon \Delta t}$
%\begin{align}
%\refp{RK_gamma_norm} \quad \Rightarrow \quad e^{\epsilon \Delta t } e^{-i\omega \Delta t}  & =  \left(1 + \sum_{\alpha=1}^{step} \gamma_{\alpha} (-ika)^\alpha (\Delta t)^\alpha \right) = \lambda \\
%\Leftrightarrow \quad \frac{w}{k} & = \arctan \left( \frac{-\text{Im}(\lambda)}{\text{Re}(\lambda)} \right)  \frac{1}{k \Delta t}
%\end{align}
%
%% fully discrete
%And in the fully discrete case, without any stabilization method we can write 
%\begin{align}
%\refp{RK_gamma0}\quad  \Rightarrow \quad U^{n+1} & = U^n + \sum_{\alpha=1}^{step} \gamma_{\alpha} A^\alpha (\Delta t)^\alpha U^n \label{RK_gamma_full} \\
%\mbox{Or} \quad \left| U^{n+1} \right| & = \left(\mathcal{I} + \sum_{\alpha=1}^{step} \gamma_{\alpha} A^\alpha (\Delta t)^\alpha\right) \left| U^n \right|  \label{RK_gamma_full_norm}  
%\end{align}
%\end{comment}

\revMR{We can now compress the problem proceeding as in the time continuous case. In  particular, using \eqref{eq_ad_fourier0} 
one easily shows that the problem can be written in terms of the local $p\times p$ matrices $\widetilde{A}:= a \widetilde{\mass}^{-1} \widetilde{\mathcal{K}_x}$ 
and in particular that
%
% $\widetilde{\mathcal{I}}$ 
%Then, using the ansatz on the shape of $U$ \eqref{eq_disp_uex1}, suggested by the Fourier analysis and Parseval's theorem, and defining $\widetilde{A}:= a \widetilde{\mass}^{-1} \widetilde{\mathcal{K}_x}$ and $\widetilde{\mathcal{I}}$ the extension to the Fourier space of the identity $\mathcal{I}$ defined in \cite{sherwin_dispersion}, we obtain for the dispersion analysis
\begin{align*}
\widetilde{\mathbf{U}}^{n+1} = G \widetilde{\mathbf{U}}^{n}\quad\text{with}\quad
G:= e^{\epsilon \Delta t } e^{-i\omega \Delta t} & \approx  \left(\widetilde{\mathcal{I}} + \sum_{j=1}^{S} \nu_{j} \Delta t^j \widetilde{A}^j \right) 
% \tildeU^{n+1} = U^{(0)} + \sum_{j=1}^{S} \nu_{j} \Delta t^jA^j  U^{(0)} = \left(\mathcal{I} + \sum_{j=1}^{S} \nu_{j}\Delta t^j A^j  \right) U^n, \label{RK_gamma0}
%\eqref{RK_gamma0} \quad \Rightarrow \quad e^{\epsilon \Delta t } e^{-i\omega \Delta t} & \approx  \left(\widetilde{\mathcal{I}} + \sum_{j=1}^{S} \nu_{j} \Delta t^j \widetilde{A}^j \right) = G,
\end{align*}}
\noindent
where $G\in \R^{p\times p}$ is the amplification matrix depending on $\theta, \Delta t$ and $ \Delta x$. Considering each eigenvalue $\lambda_i$ of $G$, we can write the following formulae for the corresponding phase $\omega_i$ and damping coefficient $\epsilon_i$
\begin{align*}
&\begin{cases}
   	e^{\epsilon_i \Delta t } \cos(\omega_i \Delta t) & = \text{Re}(\lambda_i) ,\\
   	- e^{\epsilon_i \Delta t } \sin(\omega_i \Delta t) & = \text{Im}(\lambda_i),
\end{cases}\\
\Leftrightarrow \quad & \begin{cases} 
\dfrac{\omega_i}{k} = \arctan \left( \frac{-\text{Im}(\lambda_i)}{\text{Re}(\lambda_i)} \right)  \frac{1}{k \Delta t},\\
(e^{\epsilon_i \Delta t })^2 = \text{Re}(\lambda)^2 + \text{Im}(\lambda)^2, \quad \Leftrightarrow \epsilon_i = \log\left( | \lambda_i | \right) \frac{1}{2 \Delta t}.
\end{cases}
\end{align*}
For the DeC method we can proceed with the same analysis transforming also the other involved matrices into their Fourier equivalent ones. 
Using \eqref{eq:DeCasSSPRK} these terms would contribute to the construction of $G$ not only in the $\widetilde{A}$ matrix, but also in the coefficients $\nu_j$, which become matrices as well.
At the end we just study the final matrix $G$ and its eigenstructure, whatever process was needed to build it up.

The matrix $G$ represents the evolution in one timestep of the Fourier modes for all the $p$ different types of degrees of freedom. The damping coefficients $\epsilon_i$ tell if the modes are increasing or decreasing in amplitude and the phase coefficients $\omega_i$ describe the phases of such modes.

We remark that a necessary condition for stability of the scheme is that $ |\lambda_i | \leq 1$ or, equivalently, $\epsilon_i \leq 0 $ for all the eigenvalues. The goal of our study is to find the largest CFL number for which the stability condition is fulfilled and such that the dispersion error is not too large. 
Furthermore, we notice that the matrix $G$ depends not only on $\theta, \Delta x$ and $\Delta t$, but also on at the stabilization coefficients $\tau_K$. 
Hence, the proposed analysis should contain an optimization process also along the stabilization parameter. 
\revMR{With the notation of section \S2, we will in particular set} % For ease of computation, we define a penalty coefficient $\delta$, such that the stabilization terms can be computed with the following definitions
\begin{equation*}
\begin{split}
\quad \text{SUPG :}\;\;& \tau_K =\delta  \Delta x/|a|\\[5pt]
\quad \text{LPS :} \;\;& \tau_K =\delta  \Delta x  | a |\\[5pt]
%	\item CIP : $\tau_f = \delta \mu(f)^2   |a \cdot n |$ with $n$ the outward normal of the interface (in one dimension $n=\pm1$).
\quad\text{CIP :}   \;\;& \tau_f = \delta\Delta x^2  | a |
\end{split} %with $n$ the outward normal of the interface (in one dimension $n=\pm1$).
\end{equation*}


\revMR{One of our objectives is to explore the space of parameters (CFL,$\delta$), and propose criteria allowing to set these parameters to}
%In order to obtain an indication on which CFL and $\delta$ 
provide the most stable, least dispersive and least expensive methods.
%, we will explore, for every numerical scheme, a grid of different CFLs and $\delta$s. For each of the element (CFL$,\delta)$ of this grid, 
\revMR{A clear and natural criterion is to exclude all parameter values for which we obtain  } 
 %we will ignore all the schemes that present any unstable modes with 
a positive damping coefficient $\epsilon(\theta)>10^{-12}$ for any  value of the reduced wavenumer $\theta$ (considering the machine precision). 
For all the other points we \revMR{strategies to minimize the product error times cost.} % compute different errors to give a measure of the dispersion error, choosing $a=1$. Finally we will try to maximize the CFL in order to have cheap schemes.
We %will 
compare 3 strategies to find such best parameters couples (CFL,$\delta$). The first one just chooses the highest CFL among the stable schemes. The second one relies on the relative square error of $u$, i.\,e.,
\begin{align}
	\left[\frac{u(t)-u_{ex}(t)}{u_{ex}(t)}\right]^2= &\left[e^{\epsilon t - i t(\omega-\omega_{ex})}-1\right]^2\\
	=&\left[e^{\epsilon t}\cos(t(\omega-\omega_{ex}))-1\right]^2+\left[e^{\epsilon t}\sin(t(\omega-\omega_{ex}))\right]^2\\
	=&e^{2\epsilon t} - 2 e^{\epsilon t} \cos (t(\omega-\omega_{ex})) +1.
\end{align}
Here, we denote with $\epsilon$ and $\omega$ the damping and phase of the \textit{principal }mode.
If we suppose a small dispersion error $|\omega-\omega_{ex} |\ll 1$, we can expand the cosine in the previous formula in Taylor series at the first order of accuracy, getting
\begin{align}
	\left[\frac{u(t)-u_{ex}(t)}{u_{ex}(t)}\right]^2\approx&\underbrace{\left[e^{\epsilon t} -1\right]^2}_{\text{Damping error}} + \underbrace{e^{\epsilon t}t^2 \left[\omega- \omega_{ex}\right]^2}_{\text{Dispersion error}}.
\end{align}
Computing the error at the final time $T=1$ and over the phase domain with at least 3 points per wave $0\leq k \Delta x_p \leq \frac{2\pi}{3}$, with $\Delta x_p=\frac{\Delta x}{p}$ with $p$ the degree of the polynomials,  we obtain the following $\mathbb{L}_2$ error, setting $\Delta x_p=1$,
\begin{equation}
	\eta_u(\omega,\epsilon)^2:= \frac{3}{2\pi} \left[\int_{0}^{\frac{2\pi}{3}} (e^{\epsilon}-1 )^2 dk + \int_{0}^{\frac{2\pi}{3}} e^\epsilon(\omega-\omega_{ex})^2 dk \right],
\end{equation}
reminding that $\epsilon=\epsilon(k\Delta x,$CFL$,\delta)$ and $\omega=\omega(k,\Delta x,\CFL,\delta)$ and $\omega_{ex}=k$.

The third strategy is based on a simpler error, which is only related to the dispersion, namely,
\begin{equation}
	\eta_\omega ^2(\omega):= \int_{0}^{\frac{2\pi}{3}} \left( \frac{\omega-\omega_{ex}}{\omega_{ex}}\right)^2 dk.
\end{equation}
For these last two cases we will try to minimize such an error choosing the parameter as
\begin{equation}
	(\text{CFL}^*,\delta^*):=\arg \max_{\text{CFL}} \left\lbrace \eta(\omega(\text{CFL},\delta)),\epsilon(\text{CFL},\delta)) < \mu \min_{(\text{CFL},\delta) \text{stable}} \eta(\omega(\text{CFL},\delta),\epsilon(\text{CFL},\delta))\right\rbrace.
\end{equation}

This allows to maximize the CFL without having too dispersive methods. $\mu$ must be set in order to balance the research towards something stable but also with a small dispersion error. After having tried different value, we decide to set $\mu$ to $1.3$ as it leads the choice of the parameters to meaningful, accurate and not too restrictive results.
% The 30\% of elasticity allows to not restrict too much the research on only not dispersive methods. We tried different tolerances and this seems to better balance the two components.

Summarizing, we will find the \textit{best} parameters (CFL,$\delta$) for all possible schemes with 3 strategies:
\begin{enumerate}
	\item maximizing the CFL in the stable area,
	\item minimizing $\eta_u$ and then maximizing the CFL in the stable area,
	\item minimizing $\eta_\omega$ and then maximizing the CFL in the stable area.
\end{enumerate}

In the following we will compare all the methods with these error measures, in order to suggest the best possible schemes between the proposed ones.



==> table2.tex <==

%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{amsmath,amsfonts,amsthm,amssymb}
%\usepackage{graphicx,graphics}
%\usepackage{multirow}
%\newcommand{\R}{\mathbb R}
% \newcommand{\Z}{\mathbb Z}
% \newcommand{\B}{\mathbb B}
% \newcommand{\N}{\mathbb N}
% \newcommand{\C}{\mathbb C}
% \newcommand{\Q}{\mathbb Q}
% \newcommand{\K}{\mathbb K}
%\renewcommand{\P}{\mathbb P}
%\newcommand{\Ac}{\mathcal{A}}
%\newcommand{\PP}{\mathcal{P}}
%\newcommand{\M}{\mathcal{M}}
%\begin{document}



 
%    \begin{table}
%    \begin{center}
%   \begin{tabular}{|| c  | c || c | c | c || c | c | c ||}
%     \hline
%     \multicolumn{2}{|c|}{Element } & \multicolumn{3}{|c|}{No stabilization} & \multicolumn{3}{|c|}{SUPG} \\\hline
%     \multicolumn{2}{|c|}{ $\&$ Time scheme } & $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$& $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$\\ \hline
% %   \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Basic}}} & \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{$\&$ lag.}}}
% Basic    & RK  & 0.25 & 0.2424 & 0.06 & 0.1194 & 0.3455 & 0.06 \\
% +Lagrange                          & SSPRK                & 0.25 & 0.307 & 0.06 & 0.1194 & 0.35 & 0.06 \\ \hline
% %   \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  cub.}}} &\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{$\&$ lag.}}}
%    Cubature & RK           & 0.5 & 0.35 & 0.06 & 0.1061 & 0.35 & 0.06 \\
%         +                  & SSPRK               & 0.5 & 0.35 & 0.06 & 0.1061 & 0.35 & 0.06 \\
%       Lagrange                    & DeC    & 0.5 & 0.35 & 0.1641 & 0.7 & 0.35 & 0.1 \\ 
%      %\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Basic}}}& \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{$\&$ bern.}}} & RK  & 0.25 & 0.1212 & 0.1296 & 0.1194 & 0.1728 & 0.1296 & 0.4125 & 0.1728 & 0.1258 & 0.5541 & 0.1535 & 0.1296  \\ 
%    %                    &   & SSPRK              & 0.25 & 0.1535 & 0.1296 & 0.1194 & 0.175 & 0.1458 & 0.4125 & 0.175 & 0.1502 & 0.5541 & 0.175 & 0.1458   \\ \hline                            
%                          \hline
%\multicolumn{2}{|c|}{Element } & \multicolumn{3}{|c|}{LPS} & \multicolumn{3}{|c|}{CIP}\\\hline
%     \multicolumn{2}{|c|}{ $\&$ Time scheme } & $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$& $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$\\ \hline
% %   \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Basic}}} & \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{$\&$ lag.}}} 
% Basic   & RK  &  0.4125 & 0.3455 & 0.06 & 0.5541 & 0.307 & 0.06   \\ 
%  +Lagrange                         & SSPRK      &           0.4125 & 0.35 & 0.06 & 0.5541 & 0.35 & 0.06    \\ \hline 
% %   \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  cub.}}} &\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{$\&$ lag.}}} 
%Cubat.    & RK           &  0.7667 & 0.35 & 0.06 & 0.7017 & 0.35 & 0.06   \\ 
%  +                         & SSPRK               & 0.7667 & 0.35 & 0.06 & 0.7017 & 0.35 & 0.06 \\
% Lagrange                          & DeC  &   0.9713 & 0.35 & 0.2285 & 0.8644 & 0.35 & 0.2285      \\  \hline
%
%   \end{tabular}
%   \end{center}
%    \caption{Summary table of CFL  } \label{tab:advection1D_cfl}
%
%    \end{table}
%    %
\begin{table}[h]
\begin{center}
   \begin{tabular}{| c | c || c | c | c || c | c | c | c ||c | c | c |}
     \hline
     \multicolumn{2}{|c|}{Element } & \multicolumn{3}{|c|}{No stabilization} & \multicolumn{3}{|c|}{SUPG} \\\hline
     \multicolumn{2}{|c|}{ $\&$ Time scheme } & $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$& $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$\\ \hline
%    \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Basic}}} & \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{$\&$ lag.}}} 
  Basic  & RK    & 1.58 & 1.96 & 3.78 & 1.96 & 2.95 & 3.7 \\
    +Lagrange                      & SSPRK            & 1.58 & 1.96 & 3.78 & 1.96 & 2.97 & 3.71 \\ \hline
 %   \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  cubature}}} &\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{$\&$ Lagrange}}} 
    Cubature& RK           & 1.92 & 1.99 & 3.69 & 1.96 & 2.96 & 3.73 \\
      +                     & SSPRK                & 1.92 & 1.99 & 3.7 & 1.96 & 2.96 & 3.73 \\
     Lagrange                     & DeC   & 1.99 & 1.99 & 3.61 & 2.15 & 2.4 & 3.72 \\ \hline
                         
     \multicolumn{2}{|c|}{Element } & \multicolumn{3}{|c|}{LPS} & \multicolumn{3}{|c|}{CIP}\\ \hline
     \multicolumn{2}{|c|}{ $\&$ Time scheme } & $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$& $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$\\ \hline
 %   \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Basic}}} & \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{$\&$ lag.}}} 
 Basic   & RK    & 1.96 & 2.94 & 3.71 & 1.95 & 2.94 & 3.69  \\ 
   +Lagrange                        & SSPRK             & 1.96 & 2.9 & 3.72 & 1.95 & 2.82 & 3.7   \\ \hline 
%    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  cubature}}} &\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{$\&$ lagrange}}}
Cubature     & RK           & 1.96 & 2.89 & 3.72 & 1.94 & 2.93 & 3.72   \\ 
+  & SSPRK                & 1.96 & 2.92 & 3.73 & 1.94 & 2.92 & 3.73   \\
Lagrange & DeC    & 1.99 & 2.99 & 3.75 & 1.98 & 2.98 & 3.75   \\  \hline

    %\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Basic}}}& \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{$\&$ bern.}}} & RK   & 1.58 & 1.9 & 3.61 & 1.96 & 2.97 & 3.61 & 1.96 & 3.0 & 3.63 & 1.95 & 3.0 & 3.61   \\ 
   %                     &   & SSPRK                  & 1.58 & 1.9 & 3.62 & 1.96 & 2.97 & 3.62 & 1.96 & 3.02 & 3.63 & 1.95 & 3.01 & 3.61   \\ \hline                            
   \end{tabular}
   \end{center}
    \caption{Summary table of convergence order} \label{tab:advection1D_order}
    \end{table}%    




%\begin{center}
%   \begin{tabular}{| l l l || c | c | c || c | c | c || c | c | c ||c | c | c |}
%     \hline
%     \multicolumn{15}{|c|}{Convergence order - comparison of stabilization methods}\\ \hline
%     %\multirow{2}{*}{ \backslashbox{Time scheme}{Element} }& & \multicolumn{3}{|c|}{Without any} & \multicolumn{3}{|c|}{SUPG} & \multicolumn{3}{|c|}{LPS} & \multicolumn{3}{|c|}{CIP}\\ \cline{3-14}
%     \multicolumn{3}{|c|}{Element } & \multicolumn{3}{|c|}{No stabilization} & \multicolumn{3}{|c|}{SUPG} & \multicolumn{3}{|c|}{LPS} & \multicolumn{3}{|c|}{CIP}\\ \cline{4-15}
%     \multicolumn{3}{|c|}{ $\&$ Time scheme } & $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$& $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$& $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$ & $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$ \\ \hline
%    \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Basic}}} & \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{$\&$ lag.}}} & RK    & 1.58 & 1.96 & 3.78 & 1.96 & 2.95 & 3.7 & 1.96 & 2.94 & 3.71 & 1.95 & 2.94 & 3.69  \\ 
%                         &  & SSPRK            & 1.58 & 1.96 & 3.78 & 1.96 & 2.97 & 3.71 & 1.96 & 2.9 & 3.72 & 1.95 & 2.82 & 3.7   \\ \hline 
%    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  cubature}}} &\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{$\&$ lagrange}}} & RK           & 1.92 & 1.99 & 3.69 & 1.96 & 2.96 & 3.73 & 1.96 & 2.89 & 3.72 & 1.94 & 2.93 & 3.72   \\ 
%                         &  & SSPRK                & 1.92 & 1.99 & 3.7 & 1.96 & 2.96 & 3.73 & 1.96 & 2.92 & 3.73 & 1.94 & 2.92 & 3.73   \\
%                         &  & DeC   & 1.99 & 1.99 & 3.61 & 2.15 & 2.4 & 3.72 & 1.99 & 2.99 & 3.75 & 1.98 & 2.98 & 3.75   \\  \hline
%    %\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Basic}}}& \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{$\&$ bern.}}} & RK   & 1.58 & 1.9 & 3.61 & 1.96 & 2.97 & 3.61 & 1.96 & 3.0 & 3.63 & 1.95 & 3.0 & 3.61   \\ 
%   %                     &   & SSPRK                  & 1.58 & 1.9 & 3.62 & 1.96 & 2.97 & 3.62 & 1.96 & 3.02 & 3.63 & 1.95 & 3.01 & 3.61   \\ \hline                            
%   \end{tabular}
%   \end{center}

%\end{document}

==> tables.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{amsmath,amsfonts,amsthm,amssymb}
%\usepackage{graphicx,graphics}
%\usepackage{multirow}
%\newcommand{\R}{\mathbb R}
% \newcommand{\Z}{\mathbb Z}
% \newcommand{\B}{\mathbb B}
% \newcommand{\N}{\mathbb N}
% \newcommand{\C}{\mathbb C}
% \newcommand{\Q}{\mathbb Q}
% \newcommand{\K}{\mathbb K}
%\renewcommand{\P}{\mathbb P}
%\newcommand{\Ac}{\mathcal{A}}
%\newcommand{\PP}{\mathcal{P}}
%\newcommand{\M}{\mathcal{M}}
%\begin{document}
%      
% CFL
%
\begin{table}[h]
	\begin{center}
		\begin{tabular}{| c | c || c | c | c || c |c | c | }
	     \hline
	     \multicolumn{2}{|c||}{Element } & \multicolumn{3}{|c||}{No stabilization} & \multicolumn{3}{|c|}{SUPG} \\ \hline
	     \multicolumn{2}{|c||}{ $\&$ Time scheme } & $p=1$ & $p=2$ & $p=3$ &$p=1$ & $p=2$ & $p=3$\\
	     \hline \hline
	     	% lagrange basic
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Basic}}} & RK        & 0 & 0.2424 & 0.3888    & 0.0661 & 0.07444 & 0.1914      \\
		    & SSPRK & 0 & 0.307 & 0.3888   & 0.0661 & 0.1 & 0.2424  \\
		    & DeC& 0 & 0 & 0   &    /&/&/  \\ \hline
			% lagrange cubature 
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Cub.}}} & RK          & 0 & 0.4924 & 0.4924    & 0.0588 & 0.4375 & 0.1194  \\
		    & SSPRK         & 0 & 0.4924 & 0.4924    & 0.0588 & 0.4924 & 0.1701   \\
		    & DeC        &  0 & 0.4924 & 0.4924    &    /&/&/ \\ \hline
		    % bernstein basic
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Bern.}}} & RK            &   0 &  0.1 & 0.3162 &          0.1211 & 0 & 0 \\
		     & SSPRK      & 0 & 0.1258 & 0.3981 &    0.1778 & 0 &  0 \\
		     & DeC        & 0 & 0 & 0 &  /&/&/ \\
	    \hline \hline
		%
	    \multicolumn{2}{|c||}{Element } & \multicolumn{3}{|c||}{LPS} & \multicolumn{3}{|c|}{CIP} \\ \hline
	     \multicolumn{2}{|c||}{ $\&$ Time scheme } & $p=1$ & $p=2$ & $p=3$& $p=1$ & $p=2$ & $p=3$\\
	     \hline \hline
	     	% lagrange basic
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Basic}}} & RK        & 0.4125 & 0.1304 & 0.1859                     &   0.538 & 0.1652 & 0.1914     \\
			& SSPRK   & 0.4125 & 0.1859 & 0.2219       & 0.538 & 0.2219 & 0.2219    \\
			& DeC&    0.1778 & 0.04641 & 0 &      0.2610 & 0.2610 & 0  \\ \hline
			% lagrange cubature 			
			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Cub.}}} & RK             & 0.6813 & 0.4781 & 0.1468 & 0.6236 & 0.4642 & 0.1061  \\
			& SSPRK       &  0.6813 & 0.538 & 0.1859 & 0.6236 & 0.538 & 0.1425    \\
			& DeC         &    0.6812  & 0.4641 & 0.2154 &    0.6812 & 0.4641 & 0.1467 \\ \hline
		    % bernstein basic			
			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Bern.}}} & RK            &   0.3831 & 0 & 0 &           0.4641 & 0.1211 & 0.1778\\
			& SSPRK      & 0.5623 & 0 & 0  &     0.6812 & 0.3162 & 0.2154\\
			& DeC        & 0.1778 & 0 & 0 &                    0.2610 &  0.01778 & 0.04641 \\
		\hline   
		\end{tabular}
	\end{center}
	\caption{Summary table of optimized CFL} \label{tab:dispersion_cfl}
\end{table}%
%      
% Penalty coefficient        
%
\begin{table}[h]
	\begin{center}
		\begin{tabular}{| l|  c || c | c | c |}
			\hline
			\multicolumn{2}{|c||}{Element } &   \multicolumn{3}{|c|}{SUPG}\\ \hline
			\multicolumn{2}{|c||}{ $\&$ Time scheme } &  $p=1$ & $p=2$ & $p=3$\\ \hline
	     		% lagrange basic
				\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Basic}}} & RK  & 0.3455 & 0.008377 & 0.08376   \\ 
				& SSPRK        &  0.3455 & 0.008377 & 0.1    \\ \hline 
				% lagrange cubature 			
				\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\centering  Cub.}}} & RK  & 1.3043 & 0.1557 & 0.3162   \\ 
				& SSPRK             & 1.3043 & 0.2218 & 0.3162   \\ \hline    
		    	% bernstein basic			
				\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\centering  Bern.}}} & RK  & 0.1 & 0.00001 & 0.003162    \\ 
				& SSPRK             & 0.1 & 0.00001 & 0.003162   \\  \hline
		\end{tabular}
	\end{center}
	\begin{center}
	    \begin{tabular}{| c | c || c | c | c || c |c | c |  }
	     \hline
	     \multicolumn{2}{|c||}{Element } &  \multicolumn{3}{|c||}{LPS} & \multicolumn{3}{|c|}{CIP} \\ \hline
	     \multicolumn{2}{|c||}{ $\&$ Time scheme } & $p=1$ & $p=2$ & $p=3$&  $p=1$ & $p=2$ & $p=3$  \\ \hline
	     	% lagrange basic
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Basic}}} & RK & 0.106082 & 0.2980 & 0.07896 & 0.02285 & 0.01425 & 0.003455   \\ 
		    & SSPRK      &  0.1060 & 0.2980 & 0.1229 & 0.0228 & 0.01425 & 0.005541  \\ 
		    & DeC    &      1 & 0.1778 &/                    & 0.1778  & 0.1778 & / \\ \hline 
			% lagrange cubature 			
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Cub.}}} & RK           & 0.1914 & 0.1193 & 0.03665 & 0.04641 & 0.005541 & 0.001701   \\ 
		     & SSPRK           & 0.1914 & 0.01603 & 0.03665 & 0.04641 & 0.001343 & 0.001701  \\
		     & DeC          &     0.1778 & 0.00001 & 0.03162 &     0.05623 & 0.00001 & 0.001778  \\    \hline 		     
		    % bernstein basic			
		     \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Bern.}}} & RK         &    0.1 & / & / &     0.01778 & 0.01 & 0.001778  \\ 
		     & SSPRK           &    0.1 & / & / &     0.01778 & 0.01778 & 0.001778  \\
		     & DeC         & 1  & / & / &                     0.1778  & 0.003162 & 0.001778 \\  \hline
	   \end{tabular}
   \end{center}
	\caption{Summary table of optimized penalty coefficients $\tau$} \label{tab:dispersion_penalty}
\end{table}%

==> tablesDavide.tex <==
%\documentclass{article}
%\usepackage{fullpage}
%\usepackage{amsmath,amsfonts,amsthm,amssymb}
%\usepackage{graphicx,graphics}
%\usepackage{multirow}
%\newcommand{\R}{\mathbb R}
% \newcommand{\Z}{\mathbb Z}
% \newcommand{\B}{\mathbb B}
% \newcommand{\N}{\mathbb N}
% \newcommand{\C}{\mathbb C}
% \newcommand{\Q}{\mathbb Q}
% \newcommand{\K}{\mathbb K}
%\renewcommand{\P}{\mathbb P}
%\newcommand{\Ac}{\mathcal{A}}
%\newcommand{\PP}{\mathcal{P}}
%\newcommand{\M}{\mathcal{M}}
%\begin{document}
%      
% CFL
%
\begin{table}[h]
	\begin{center}
		\begin{tabular}{| c | c || c | c | c || c |c | c | }
	     \hline
	     \multicolumn{2}{|c||}{Element } & \multicolumn{3}{|c||}{No stabilization} & \multicolumn{3}{|c|}{SUPG} \\ \hline
	     \multicolumn{2}{|c||}{ $\&$ Time scheme } & $p=1$ & $p=2$ & $p=3$ &$p=1$ & $p=2$ & $p=3$\\
	     \hline \hline
	     	% lagrange basic
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Basic}}} & RK       & 0 & 0.316228 & 0.199526       & 0.429193 & 0.188586 & 0.238534     \\
		    & SSPRK   & 0 & 0.316228 & 0.199526    & 0.61054 & 0.238534 & 0.238534 \\
		    & DeC       & 0 & 0 & 0                    & 0.686649 & 0.1      & 0.0364103   \\ \hline
			% lagrange cubature 
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Cub.}}} & RK        & 0. & 0.398107 & 0.316228         & 0.868511 & 0.301711 & 0.238534    \\
		    & SSPRK        & 0. & 0.398107 & 0.316228      & 0.976778 & 0.339322 & 0.26827   \\
		    & DeC       & 0. & 0.398107 & 0.251189        & 0.381621 & 0.381621 & 0.26827    \\ \hline
		    % bernstein basic
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Bern.}}} & RK         & 0. & 0.316228 & 0.199526     & 0.429193 & 0.188586 & 0.238534 \\
		     & SSPRK       & 0. & 0.316228 & 0.199526  & 0.61054 & 0.238534 & 0.238534  \\
		     & DeC          & 0 & 0 & 0                   & 0.686649 & 0.0381621 & 0.238534    \\
	    \hline \hline
		%
	    \multicolumn{2}{|c||}{Element } & \multicolumn{3}{|c||}{LPS} & \multicolumn{3}{|c|}{CIP} \\ \hline
	     \multicolumn{2}{|c||}{ $\&$ Time scheme } & $p=1$ & $p=2$ & $p=3$& $p=1$ & $p=2$ & $p=3$\\
	     \hline \hline
	     	% lagrange basic
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Basic}}} & RK        & 0.429193 & 0.188586 & 0.238534   & 0.482696 & 0.188586 & 0.238534      \\
			& SSPRK     & 0.61054 & 0.238534 & 0.238534    & 0.686649 & 0.238534 & 0.238534    \\
			& DeC       & 0.429193 & 0.238534 & /          & 0.542868 & 0.212095 & /    \\ \hline
			% lagrange cubature 			
			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Cub.}}} & RK          & 0.976778 & 0.482696 & 0.26827    & 0.976778 & 0.482696 & 0.26827    \\
			& SSPRK      & 1.23548 & 0.482696 & 0.26827     & 1.23548 & 0.482696 & 0.26827    \\
			& DeC         & 0.976778 & 0.482696 & 0.26827    & 0.976778 & 0.482696 & 0.26827   \\ \hline
		    % bernstein basic			
			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Bern.}}} & RK        & 0.429193 & 0.188586 & 0.238534   & 0.482696 & 0.188586 & 0.238534   \\
			& SSPRK      & 0.61054 & 0.238534 & 0.238534    & 0.686649 & 0.238534 & 0.238534     \\
			& DeC         & 0.429193 & 0.0582514 & 0.117877  & 0.542868 & 0.0655129 & 0.117877  \\
		\hline   
		\end{tabular}
	\end{center}
	\caption{Summary table of optimized CFL} \label{tab:dispersion_cfl}
\end{table}%

%      
% CFL
%
\begin{table}[h]
	\begin{center}
		\begin{tabular}{| c | c || c | c | c || c |c | c | }
			\hline
			\multicolumn{2}{|c||}{Element } & \multicolumn{3}{|c||}{No stabilization} & \multicolumn{3}{|c|}{SUPG} \\ \hline
			\multicolumn{2}{|c||}{ $\&$ Time scheme } & $p=1$ & $p=2$ & $p=3$ &$p=1$ & $p=2$ & $p=3$\\
			\hline \hline
			% lagrange basic
			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Basic}}} & RK      & 0. & 0.398107 & 0.316228    & 0.542868 & 0.482696 & 0.381621     \\
			& SSPRK & 0. & 0.501187 & 0.398107    & 0.772245 & 0.61054 & 0.429193  \\
			& DeC     & 0 & 0    &   0              & 1.75751 & 0.482696 & 0.0429193   \\ \hline
			% lagrange cubature 
			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Cub.}}} & RK         & 0 & 0.501187 & 0.501187     & 0.976778 & 0.686649 & 0.482696  \\
			& SSPRK         &  0 & 0.630957 & 0.501187     & 1.3895 & 0.772245 & 0.542868   \\
			& DeC       & 0 & 0.501187 & 0.501187     & 1.56271 & 0.976778 & 0.61054   \\ \hline
			% bernstein basic
			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Bern.}}} & RK         & 0 & 0.398107 & 0.316228     & 0.542868 & 0.482696 & 0.381621 \\
			& SSPRK      & 0 & 0.501187 & 0.398107     & 0.772245 & 0.61054 & 0.429193  \\
			& DeC         & 0   &0 & 0                  & 1.75751 & 0.976778 & 0.686649  \\
			\hline \hline
			%
			\multicolumn{2}{|c||}{Element } & \multicolumn{3}{|c||}{LPS} & \multicolumn{3}{|c|}{CIP} \\ \hline
			\multicolumn{2}{|c||}{ $\&$ Time scheme } & $p=1$ & $p=2$ & $p=3$& $p=1$ & $p=2$ & $p=3$\\
			\hline \hline
			% lagrange basic
			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Basic}}} & RK       & 0.542868 & 0.482696 & 0.381621   & 0.686649 & 0.542868 & 0.381621     \\
			& SSPRK    & 0.868511 & 0.61054 & 0.429193    & 1.09854 & 0.61054 & 0.429193     \\
			& DeC      & 0.482696 & 0.542868 & /          & 0.772245 & 0.61054 & /     \\ \hline
			% lagrange cubature 			
			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Cub.}}} & RK            & 0.976778 & 0.686649 & 0.482696   & 0.976778 & 0.686649 & 0.482696    \\
			& SSPRK      & 1.3895 & 0.868511 & 0.61054      & 1.3895 & 0.868511 & 0.61054   \\
			& DeC         & 0.976778 & 0.686649 & 0.482696   & 0.976778 & 0.686649 & 0.482696 \\ \hline
			% bernstein basic			
			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Bern.}}} & RK          & 0.542868 & 0.482696 & 0.381621   & 0.686649 & 0.542868 & 0.381621 \\
			& SSPRK      & 0.868511 & 0.61054 & 0.429193    & 1.09854 & 0.61054 & 0.429193  \\
			& DeC         & 0.482696 & 0.0582514 & 0.117877  & 0.772245 & 0.0655129 & 0.117877  \\
			\hline   
		\end{tabular}
	\end{center}
	\caption{Summary table of maximum CFL to get stability} \label{tab:dispersion_cfl_ever}
\end{table}%
%      
% Penalty coefficient        
%
\begin{table}[h]
	\begin{center}
		\begin{tabular}{| l|  c || c | c | c |}
			\hline
			\multicolumn{2}{|c||}{Element } &   \multicolumn{3}{|c|}{SUPG}\\ \hline
			\multicolumn{2}{|c||}{ $\&$ Time scheme } &  $p=1$ & $p=2$ & $p=3$\\ \hline
	     		% lagrange basic
				\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Basic}}} & RK   & 0.125893 & 0.00794328 & 0.0199526   \\  
				& SSPRK        & 0.125893 & 0.00630957 & 0.0251189    \\ 
				& DeC       & 0.501187 & 0.00158489 & 0.0199526   \\ \hline 
				% lagrange cubature 			
				\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\centering  Cub.}}} & RK & 0.398107 & 0.316228 & 0.158489   \\ 
				& SSPRK            & 0.501187 & 0.398107 & 0.0794328  \\ 
				& DeC        & 0.630957 & 0.0158489 & 0.0501187  \\ \hline     
		    	% bernstein basic			
				\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\centering  Bern.}}} & RK  & 0.125893 & 0.00794328 & 0.0199526    \\ 
				& SSPRK             & 0.125893 & 0.00630957 & 0.0251189 \\ 
				& DeC        & 0.501187 & 0.0316228 & 0.1    \\ \hline 
		\end{tabular}
	\end{center}
	\begin{center}
	    \begin{tabular}{| c | c || c | c | c || c |c | c |  }
	     \hline
	     \multicolumn{2}{|c||}{Element } &  \multicolumn{3}{|c||}{LPS} & \multicolumn{3}{|c|}{CIP} \\ \hline
	     \multicolumn{2}{|c||}{ $\&$ Time scheme } & $p=1$ & $p=2$ & $p=3$&  $p=1$ & $p=2$ & $p=3$  \\ \hline
	     	% lagrange basic
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Basic}}} & RK & 0.158489 & 0.00794328 & 0.0251189   & 0.0199526 & 0.000398107 & 0.000630957     \\ 
		    & SSPRK       & 0.158489 & 0.00630957 & 0.0398107   & 0.0199526 & 0.000398107 & 0.001     \\ 
		    & DeC        & 1 & 0.0630957 & /                   & 0.125893 & 0.00316228 & /     \\ \hline 
			% lagrange cubature 			
		    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Cub.}}} & RK          & 0.501187 & 0.125893 & 0.0316228     & 0.125893 & 0.0125893 & 0.00125893   \\ 
		     & SSPRK         &   0.398107 & 0.158489 & 0.0501187     & 0.1 & 0.0125893 & 0.00199526      \\
		     & DeC         & 0.501187 & 0.125893 & 0.0316228     & 0.125893 & 0.0125893 & 0.00125893   \\    \hline 		     
		    % bernstein basic			
		     \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Bern.}}} & RK         & 0.158489 & 0.00794328 & 0.0251189   & 0.0199526 & 0.000398107 & 0.000630957    \\ 
		     & SSPRK          & 0.158489 & 0.00630957 & 0.0398107   & 0.0199526 & 0.000398107 & 0.001    \\
		     & DeC           & 1 & 0.199526 & 0.199526             & 0.125893 & 0.0125893 & 0.00794328 \\  \hline
	   \end{tabular}
   \end{center}
	\caption{Summary table of optimized penalty coefficients $\tau$} \label{tab:dispersion_penalty}
\end{table}%


%      
% Penalty coefficient for best CFL  stable schemes (no dispersion)
%
\begin{table}[h]
	\begin{center}
		\begin{tabular}{| l|  c || c | c | c |}
			\hline
			\multicolumn{2}{|c||}{Element } &   \multicolumn{3}{|c|}{SUPG}\\ \hline
			\multicolumn{2}{|c||}{ $\&$ Time scheme } &  $p=1$ & $p=2$ & $p=3$\\ \hline
			% lagrange basic
			\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Basic}}} & RK  & 1.25893 & 0.316228 & 6.30957     \\  
			& SSPRK       & 0.0199526 & 5.01187 & 0.00199526    \\ 
			& DeC      & 1.58489 & 0.0794328 & 0.0630957   \\ \hline 
			% lagrange cubature 			
			\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\centering  Cub.}}} & RK & 0.0398107 & 0.00794328 & 0.794328  \\ 
			& SSPRK           & 0.158489 & 0.158489 & 0.00125893 \\ 
			& DeC        & 0.630957 & 0.000251189 & 39.8107 \\ \hline     
			% bernstein basic			
			\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\centering  Bern.}}} & RK  & 1.25893 & 0.316228 & 6.30957     \\ 
			& SSPRK           & 0.0199526 & 5.01187 & 0.00199526  \\ 
			& DeC         & 1.58489 & 0.199526 & 0.0501187   \\ \hline 
		\end{tabular}
	\end{center}
	\begin{center}
		\begin{tabular}{| c | c || c | c | c || c |c | c |  }
			\hline
			\multicolumn{2}{|c||}{Element } &  \multicolumn{3}{|c||}{LPS} & \multicolumn{3}{|c|}{CIP} \\ \hline
			\multicolumn{2}{|c||}{ $\&$ Time scheme } & $p=1$ & $p=2$ & $p=3$&  $p=1$ & $p=2$ & $p=3$  \\ \hline
			% lagrange basic
			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Basic}}} & RK  & 1.25893 & 0.316228 & 6.30957         & 2.51189 & 0.000158489 & 6.30957      \\ 
			& SSPRK       & 1.25893 & 0.01 & 0.794328            & 0.1 & 0.00251189 & 0.0398107     \\ 
			& DeC       & 1.99526 & 3.16228 & /                & 0.630957 & 0.000199526 & /        \\ \hline 
			% lagrange cubature 			
			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Cub.}}} & RK         & 0.0398107 & 0.00794328 & 0.794328    & 2.51189 & 0.000630957 & 0.000501187      \\ 
			& SSPRK         & 6.30957 & 0.00501187 & 0.000630957   & 5.01187 & 1.25893 & 0.00501187        \\
			& DeC        & 0.0398107 & 0.00794328 & 0.794328    & 2.51189 & 0.000630957 & 0.000501187    \\    \hline 		     
			% bernstein basic			
			\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Bern.}}} & RK           & 1.25893 & 0.316228 & 6.30957         & 2.51189 & 0.000158489 & 6.30957   \\ 
			& SSPRK          & 1.25893 & 0.01 & 0.794328            & 0.1 & 0.00251189 & 0.0398107     \\
			& DeC           & 1.99526 & 0.000794328 & 0.000398107  & 0.630957 & 2.51189 & 0.00199526  \\  \hline
		\end{tabular}
	\end{center}
	\caption{Summary table of optimized penalty coefficients $\tau$} \label{tab:dispersion_penalty_Ever}
\end{table}%
